An Unsupervised C-Uniform Trajectory Sampler with Applications to Model Predictive Path Integral Control

Sampling-based model predictive controllers generate trajectories by sampling control inputs from a fixed, simple distribution such as the normal or uniform distributions. This sampling method yields trajectory samples that are tightly clustered around a mean trajectory. This clustering behavior in turn, limits the exploration capability of the controller and reduces the likelihood of finding feasible solutions in complex environments. Recent work has attempted to address this problem by either reshaping the resulting trajectory distribution or increasing the sample entropy to enhance diversity and promote exploration. In our recent work, we introduced the concept of C-Uniform trajectory generation [1] which allows the computation of control input probabilities to generate trajectories that sample the configuration space uniformly. In this work, we first address the main limitation of this method: lack of scalability due to computational complexity. We introduce Neural C-Uniform, an unsupervised C-Uniform trajectory sampler that mitigates scalability issues by computing control input probabilities without relying on a discretized configuration space. Experiments show that Neural C-Uniform achieves a similar uniformity ratio to the original C-Uniform approach and generates trajectories over a longer time horizon while preserving uniformity. Next, we present CU-MPPI, which integrates Neural C-Uniform sampling into existing MPPI variants. We analyze the performance of CU-MPPI in simulation and real-world experiments. Our results indicate that in settings where the optimal solution has high curvature, CU-MPPI leads to drastic improvements in performance.

==> sections/background.tex <==
\section{Preliminaries}

In this section, we summarize important definitions, dynamic model and concepts required to develop our approach.


% \vtxt{the model is also presented in the experiments section IV. B. Unless you are considering multiple sytems you can merge the two. Here say you are using a state space representation. And then give the specific model as an example}
We consider a robotic system with a state $\statevec \in \mathcal{X} \subseteq \mathcal{R}^p$, and a control input $u \in \mathcal{U} \subseteq \mathcal{R}^q$ with the known discrete dynamic model $\statevec_{t+1} = \mathbf{F}(\statevec_t, u_t)$. We use the dubin's car as our dynamic model where $\statevec = [x,y, \psi] \in \mathbb{R}^3 $ is the vehicle's state and $u = \omega$ is the angular velocity. The state transition is defined using Equation \ref{eq;kinematic_model}.

\begin{align}   \label{eq;kinematic_model}
    \dot{\statevec} &= \mathbf{F}(\statevec, u) = 
    \begin{bmatrix}
        \dot{x} \\
        \dot{y} \\
        \dot{\psi}
    \end{bmatrix}
    =
    \begin{bmatrix}
        v\cos\psi \\
        v\sin\psi \\
        \omega
    \end{bmatrix}
\end{align}

We also define finite horizon trajectories with horizon $T$ as $\tau = \mathbf{F}(\statevec_0, \mathbf{U})$, where $\statevec_0$ is the initial state, and $\mathbf{U} =(u_0, u_1, \dots, u_{T-1})$ is the control sequence. The resulting trajectory $\tau$ is generated by recursively applying $F$ with corresponding state $\statevec_t$ and control $u_t$ pairs. It is assumed that the dynamic model $F$ satisfies the Lipschitz continuity, which means the state propagation with this model is predictable.

We define a \textit{Level Set} $L_t$ as the following equation:
\begin{equation}
L_t = \{ \mathbf{x} \in \mathcal{X} \ | \ \exists \mathbf{U} = (u_0, u_1, \dots, u_{t-1}) \text{ s.t. } \mathbf{x} = F(\statevec_0, \mathbf{U}) \}.
\end{equation}
% \vtxt{``denote" means you are giving notation. maybe you mean "we note.."}
where set of all states $\mathbf{x} \in \mathcal{X}$ such that there is a control sequence $\mathbf{U}$ of length $t$ with $\statevec = F(\statevec_0, \mathbf{U})$. We also need to note that these level sets are disjoint, meaning if a state $\statevec_i$ is already covered by some $L_i$, we discard that state that is also reachable in any later level set $L_j$, where $j > i$. Lastly, we define $L_{D,t}$ as the discretized version of $L_{t}$ where each state $\statevec_{D,t} \in L_{D,t}$ is found as $L_{t}/\delta$ where $\delta$ defines a small measurable uniform region of \ourmethod. 

The probabilities associated with level sets are computed recursively for each level set as follows. 

% \begin{equation}
% p(\statevec') = \sum_{\statevec \in L} \sum_{u: \statevec'= F(\statevec, u) } p(u|\statevec)p(\statevec)
% \label{eqn:lprobs}
% \end{equation}

\begin{equation}
p(\statevec_{t+1}) = \sum_{\statevec_t \in L_t} \sum_{\mathbf{u_i}: \statevec_{t+1}= F(\statevec_t, \mathbf{u_i}) } p(u_i|\statevec_t)p(\statevec_t)
\label{eqn:lprobs}
\end{equation}

% where $\statevec'$ is the state in the next level set.
where $\statevec_{t+1}$ is the state in the next level set. The uniform probability of a state within a given level set $p(\statevec_t), \statevec \in L_t$  can be determined by the ratio of the measure of an infinitesimal measurable region ($\delta$) to the total measure of the level set. We use the Lebesgue measure ($\mu$) to quantify the size of these spaces as stated in \cite{poyrazoglu2024cuniformtrajectorysamplingfast}. Besides that, we discretize the action space $\mathcal{U}$ into a set of distinct actions $\mathcal{U} = \{u_0,u_1,\dots,u_N\}$ and we define probability mass function (pmf) over it. The pmf is denoted as $p(\mathcal{U}|\statevec)$, where $\sum_{i=0}^N p(u_i|\statevec) = 1$, and $p(u_i|\statevec) \geq 0$. 


% \vtxt{i would define what these probabilities are. 
% When you do that you will see that (1) you need to provide $u$ as input or say it's fixed or something and (2) define a pdf over the u first -- i.e the first term of the product. Then you can say something like: "give a control sequence pdf $p(u, x)$ for level set i, the probability that the robot is in state $x \in L_{i+1}$ is ...}

By introducing the Eq.~\ref{eqn:lprobs}, we use a similar problem formulation as defined in~\cite{poyrazoglu2024cuniformtrajectorysamplingfast}: 


Given an initial state $\statevec_0$ and a system's dynamic model $F$ determine control action probabilities $p(\mathcal{U}|\statevec)$ for each state such that the probability distribution associated with each level-set is uniform.




==> sections/background_iros_long.tex <==
\section{Preliminaries}



In this section, we summarize important definitions, dynamic models, and concepts required to develop our approach. After these definitions, we first explain what \ourmethod{} trajectories are in Sec.~\ref{sec:cuniform_traj_samp}, and then we also review the general sampling-based model predictive controller problem formulation by explaining the MPPI algorithm in Sec.~\ref{sec:sbmpc_pre}.

\begin{figure*}[!ht]
    \centering
    \subfloat[MPPI]{\includegraphics[width=0.18\textwidth, height = 3cm]{Figures/env_2.png}}
    \hfill
    \subfloat[SVG-MPPI]{\includegraphics[width=0.18\textwidth, height = 3cm]{Figures/env_1.png}}
    \hfill
    \subfloat[\newsampourmethod]{\includegraphics[width=0.18\textwidth, height = 3cm]{Figures/env_3.png}}
    \hfill
    \subfloat[Cost-Trajectory]{\includegraphics[width=0.25\textwidth, height = 3cm]{Figures/cost.png}}

    \caption{Drawback Illustration: MPPI and a gradient-based variant of MPPI, SVG-MPPI, get stuck in local minima as shown in Figure (a)-(b). The green trajectories represent the MPPI solution, whereas the blue trajectory represents the nominal trajectory generated by SVG. Our approach \newsampourmethod{} shown in Figure (c) utilizes the diverse trajectories of \newourmethod{} and escapes from the local minima by selecting the trajectory with the lowest cost and using it as a nominal for MPPI. Figure (d) illustrates the cost-trajectory landscape where red represents SVG-MPPI, blue represents MPPI, and green represents \newsampourmethod{}. }
    \label{fig:drawback_illustration}
\end{figure*}

We consider a robotic system with a state vector $\statevec \in \mathcal{X} \subseteq \mathcal{R}^p$, and a control input vector $\mathbf{u} \in \mathcal{U} \subseteq \mathcal{R}^q$ with the known discrete dynamic model $\statevec_{t+1} = \mathbf{F}(\statevec_t, \mathbf{u}_t)$. We use a kinematic bicycle car model as our vehicle model where $\statevec = [x,y, \psi] \in \mathbb{R}^3 $ is the vehicle's state, and $\mathbf{u} = [v, \delta]$ is the steering angle and the linear velocity $v$ is constant. The state transition is defined using Equation \ref{eq;kinematic_bicycle_model}.

\vspace{-10pt}
\begin{align}   \label{eq;kinematic_bicycle_model} 
    \statevec_{t+1} &= \mathbf{F}(\statevec_t, u) = 
    \begin{bmatrix}
        x_t \\
        y_t \\
        \psi_t
    \end{bmatrix} \Delta_t
    =
    \begin{bmatrix}
        v\cos\psi_t \\
        v\sin\psi_t \\
        \frac{v}{L_{wb}}\tan(\delta_t)
    \end{bmatrix} \Delta_t
\end{align}
where $\Delta_t$ is the time discretization.

We also define finite horizon trajectories with horizon $T$ as $\tau = \mathbf{F}(\statevec_0, \mathbf{U})$, where $\statevec_0$ is the initial state, and $\mathbf{U} =(\mathbf{u}_0, \mathbf{u}_1, \dots, \mathbf{u}_{T-1})$ is the control sequence. The resulting trajectory $\tau$ is generated by recursively applying $F$ with corresponding state $\statevec_t$ and control $\mathbf{u}_t$ pairs. It is assumed that the dynamic model $F$ satisfies the Lipschitz continuity, which means the state propagation with this model is predictable.


\subsection{C-Uniform Trajectory Sampling} \label{sec:cuniform_traj_samp}

We provide key concepts of the \ourmethod{} trajectory sampling. For more details, we direct the reader to prior research~\cite{poyrazoglu2024cuniformtrajectorysamplingfast}. We first define a \textit{Level Set} $L_t$ as the following equation:
\begin{equation}
L_t = \{ \statevec_t \in \mathcal{X} \ | \ \exists \mathbf{U}  =(\mathbf{u}_0, \mathbf{u}_1, \dots, \mathbf{u}_{t-1}) \text{ s.t. } \statevec_t = F(\statevec_0, \mathbf{U}) \}.
\end{equation}
where the set of all states $\statevec_t \in \mathcal{X}$ such that there is a control sequence $\mathbf{U}$ of length $t$ with $\statevec = F(\statevec_0, \mathbf{U})$. We also need to note that these level sets are disjoint, meaning if a state $\statevec_i$ is already covered by some $L_i$, we discard that state that is also reachable in any later level set $L_j$, where $j > i$. Lastly, we define $L_{D,t}$ as the discretized version of $L_{t}$ where each representative state $\statevec_{D,t} \in L_{D,t}$ is found by $L_{t}/\delta$ where $\delta$ defines a small measurable uniform region of \ourmethod. We use the Lebesgue measure ($\mu$) to quantify the size of these regions. Then, the uniform probability of representatives for each level set is defined as $P(\statevec_{t} \in \delta) = \mu(\delta)/\mu(L_t)$, where $\statevec_{t}$ is a state in the uniformity cell. 

The probabilities associated with level sets are computed recursively for each level set as follows. 
\vspace{-2pt}
\begin{equation}
p(\statevec_{t+1}) = \sum_{\statevec_t \in L_t} \sum_{\mathbf{u_i}: \statevec_{t+1}= F(\statevec_t, \mathbf{u_i}) } p(u_i|\statevec_t)p(\statevec_t)
\label{eqn:lprobs}
\end{equation}
where $\statevec_{t+1}$ is the state in the next level set, and the control inputs $\mathbf{u}_i$ are the ones that reach the state $\statevec_{t+1}$ by propagating the current state $\statevec_t$. Additionally, we also discretize the action space $\mathcal{U}$ into a set of distinct actions $\mathcal{U} = \{u_0,u_1,\dots,u_N\}$ and we define probability mass function (pmf) over it. The pmf is denoted as $p(\mathcal{U}|\statevec)$, where $\sum_{i=0}^N p(u_i|\statevec) = 1$, and $p(u_i|\statevec) \geq 0$. 

By introducing the Eq.~\ref{eqn:lprobs}, we can state a similar problem formulation for the \newourmethod{} trajectory sampling, as defined in~\cite{poyrazoglu2024cuniformtrajectorysamplingfast}: 

Given an initial state $\statevec_0$ and a system's dynamic model $F$ determine control action probabilities $p(\mathcal{U}|\statevec)$ for each state such that the probability distribution associated with each level set is uniform.



\subsection{Sampling-Based Model Predictive Control} \label{sec:sbmpc_pre}

We review the Information-Theoretic MPPI algorithm~\cite{williams2018information} and its formulation for sampling-based model predictive control (SBMPC).

MPPI optimizes the action sequence $\mathbf{U} = (\mathbf{u}_t, \dots, \mathbf{u}_{t+T})$ over a time horizon $T$ by minimizing the expected cost:
\vspace{-3pt}
\begin{equation}\label{eq:opt_control} \mathbf{U}_t^* = \arg\min_{\mathbf{U}_t \in \mathcal{U}} \mathbb{E}_{\mathbf{V} \sim q(V|U,\Sigma)} [ J(\statevec_t, \mathbf{V}) ]
\end{equation}
where $J(\statevec_0, \mathbf{V})$ is the cost function and the control perturbations are modeled as, $ \mathbf{v}_t = \mathbf{u}_t + \epsilon$, where $\epsilon \sim \mathcal{N}(0,\Sigma)$. To derive an optimal control policy, MPPI introduces the concept of free energy, defined as:
\vspace{-2pt}
\begin{equation} 
\mathcal{F}(S,p, \statevec_0, \lambda) = \log \mathbb{E}_{\mathbb{P}}[\exp(-S(\mathbf{V})/\lambda)] \end{equation}
where $S(\mathbf{V})$ represents the total state cost, $\lambda$ is a temperature parameter controlling exploration, and $\mathbb{P}$ is a base probability distribution. The free energy function provides a lower bound on the optimal cost function, 
\vspace{-3pt}
\begin{equation}\label{eq:lower_bound_free} -\mathcal{F}(S,p, \statevec_0, \lambda) \leq \mathbb{E}{\mathbb{Q}}[S(\mathbf{V})/\lambda] + D{KL}(\mathbb{Q}||\mathbb{P}). \end{equation}

By defining the base distribution $p(\mathbf{V})$ and the optimal control distribution $q^*(\mathbf{V})$ as:
\vspace{-3pt}
\begin{align} 
& p(\mathbf{V})  = q(\mathbf{V}|\tilde{\mathbf{U}}, \Sigma), \quad q^*(\mathbf{V}) \propto \exp(-S(\mathbf{V})/\lambda) p(\mathbf{V})
\end{align}
the optimization reduces to minimizing the KL divergence between the optimal control distribution and the current control distribution:
\vspace{-3pt}
\begin{equation}\label{eq:argmin_kl} \mathbf{U}^* = \arg\min_{\mathbf{U} \in \mathcal{U}} D_{KL}(\mathbb{Q^*}||\mathbb{Q}), \end{equation}

Through importance sampling, the optimal control sequence can be computed as a weighted expectation over sampled trajectories:
\vspace{-2pt}
\begin{equation}\label{eq:opt_u_calc} \mathbf{U}^* = \mathbb{E}_{\mathbb{Q}}[w(\mathbf{V})\mathbf{V}], \quad w(\mathbf{V}) = \frac{q^*(\mathbf{V})}{q(\mathbf{V}|\mathbf{U},\Sigma)}. \end{equation}

In practice, Monte Carlo sampling methods are used to approximate the expectation. Further details on the derivation can be found in~\cite{williams2018information}.

However, Gaussian assumptions in $p(\mathbf{V})$ and $q^*(\mathbf{V})$ limit MPPI in highly nonconvex or multimodal cost landscapes, leading to suboptimal solutions (Fig.~\ref{fig:drawback_illustration}). In those landscapes, Gaussian perturbations may fail to explore promising regions and MPPI can get stuck in local minima.


==> sections/experiments.tex <==
\section{Experiments}
% In this section, we aim to evaluate our \newourmethod{} sampling method by addressing the following questions through experiments.  
% \begin{enumerate}
%     \item Can \newourmethod{} maintain uniformity when extrapolating to a longer time horizon than it was trained on?
%     \item How well uniform trajectory sampling using the \newourmethod{} cover the C-space, and how does the  coverage performance affect the robot's navigation performance in complex environments?
%     \item Does planning with a long time horizon or finer discretization help improve the robot's ability to navigate in complex environments? \vtxt{what's the difference between 2 and 3?}
%     % \item How does the continuous representation of the C-space with \newourmethod{} compare to a discrete representation with \ourmethod{} in terms of navigation performance
% % \end{enumerate}
% We first demonstrate the uniformity analysis of \newourmethod{} in Sec.~\ref{sec: uniformity_analysis}. We then demonstrate coverage analysis to compare the \newourmethod{} with other trajectory sampling baselines in Sec.~\ref{sec: coverage_exp}. Lastly, we showcase simulation and real-world experiments designed to analyze the performance of the methods in cluttered and dynamic environment settings in Sec.~\ref{sec: simulation} and Sec.~\ref {sec: real_world_exp}.

% We mainly compare \newourmethod{} with the C-Uniform method \cite{poyrazoglu2024cuniformtrajectorysamplingfast} and other state-of-the-art baseline methods, such as MPPI \cite{williams2018information}, and log-MPPI \cite{williams2018robust}. These baseline methods are selected since they generate trajectory samples solely based on the sampling distribution without additional external optimizers being implemented to alter the distribution.


% REAL WORLD



% \begin{table*}[h]
% \centering
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% \textbf{Number of Sampled Trajectories} &\textbf{MPPI} &\textbf{log-MPPI} &\textbf{Neural C-Uniform}& \textbf{C-Uniform} \\ \hline
% 250   & --  &-- &2.35 &--\\ \hline
% 500   & -- &-- &4.15 &--\\ \hline
% 1000   & -- &-- &6.97 &--\\ \hline
% 2500   & -- &-- &13.15 &--\\ \hline
% 5000   & -- &-- &19.47 &--\\ \hline
% 10000   & -- &-- &26.95 &--\\ \hline
% 50000   & -- &-- &44.54 &--\\ \hline
% \end{tabular}
% \caption{Coverage Performance (\%)}
% \label{tab:probabilities}
% \end{table*}



% We present the uniformity analysis of \newourmethod{} to showcase the capability to sample each level set uniformly. We perform iterative uniformity analysis by checking for each $L_{D,t}$, can the network learn to sample $L_{D,t+1}$ uniformly. We use the entropy ratio to the uniform distribution as a measure to determine the uniformity of samples. Algorithm \ref{algo:uniformity_metric} shows the uniformity metric calculated per level set where $N_{L_{t+1}}$ denotes the number of states $\statevec_{D,t+1}$ in $L_{D,t+1}$ and $Occ(\statevec_{D,t+1})$ represents the count of the occurrences of $\statevec_{D,t+1}$ in $L_{D,t+1}$. We mainly perform the uniformity analysis for two settings - interpolation and extrapolation. 
% \begin{algorithm}
% \caption{Uniformity Metric} \label{algo:uniformity_metric}
% \KwIn{
%     $L_{D,t}$: Discretized C-Uniform Level Set at time $t$;\\
%     $L_{D,t+1}$: Discretized C-Uniform Level Set at time $t+1$;\\
%     $\mathcal{U}$: Set of actions;\\
%     $\Delta t$: the time step;
% }   
% \KwOut{Uniformity Metric;}
%     $Occ = \{Occ(\statevec_{D,t+1})\}_{\statevec_{D,t+1} \in L_{D,t+1}}$ 
    
%     Initialize $Occ(\statevec_{D,t+1})= 0$ for all $\statevec_{D,t+1} \in L_{D,t+1}$
    
%     \For{each cell representative $\statevec_{D,t} \in \mathcal{L}_{D,t}$}{
%             \For{each action $u \in \mathbf{U}$}{
%             $\statevec_{t+1}\leftarrow f(\statevec_{D,t}, \mathbf{u}, \Delta t)$\;

%             Determine $\statevec_{D,t+1}$ closest to $\statevec_{t+1}$ in $L_{D,t+1}$ 

%             $Occ(\statevec_{D,t+1}) \leftarrow Occ(\statevec_{D,t+1}) + p_\theta(\mathbf{u}|\statevec_{D,t})$
%         }
%     }
%     $p(\statevec_{D,t+1})$ = $Occ(\statevec_{D,t+1})/\sum_{\statevec_{D,t+1} \in L_{D,t+1}}Occ(\statevec_{D,t+1})$
    
%     $\mathcal{H} = \sum_{\statevec_{D,t+1} \in L_{D,t+1}} p(\statevec_{D,t+1}) \log p(\statevec_{D,t+1})$
    
%     $\mathcal{H}_{uniform} = \sum_{i=0}^{N_{D,L_{t+1}}} \frac{1}{N_{D,L_{t+1}}} \log \frac{1}{N_{D,L_{t+1}}}$
    
%     \Return $100 \cdot \frac{\mathcal{H}}{\mathcal{H}_{uniform}}$
% \end{algorithm}
% \subsubsection{Training}
% We evaluate the model on the training level sets to check the uniformity of the model. The training level set consisted of 4 second time horizon with 0.2 time discretization which results in 20 level sets. Figure \ref{fig:dubins_uniformity} shows the uniformity metric calculated for each level set. It can be seen that we are close to 100\% uniform over level sets. 
% \begin{figure}[!h]
%     \begin{center}
%         \includegraphics[width=0.8\columnwidth]{Figures/quantitative_analysis_NN_unsupervised.png}
%     \end{center}
%     \caption{Training Uniformity Analysis: The Figure analyzes the uniformity achieved by \newourmethod{} on the training level sets which consists of 4 second trajectory with 0.2 time discretization. It can be observed that \newourmethod{} is uniform on all level sets}
% \label{fig:dubins_uniformity}
% \end{figure}
% \subsubsection{Interpolation}
% The interpolation experiment showcases the capability of \newourmethod{} to determine controls at a higher frequency. We demonstrate it by training \newourmethod{} on 4 second time horizon with 0.4 time discretization while testing it with 0.2 time discretization. Figure \ref{fig:dubins_uniformity_analysis} (blue) shows the uniformity metric calculated for each level set for the interpolation experiment where the x-axis showcase the level sets for 6 seconds horizon with 0.2 discretization while the y-axis shows the uniformity metric performance. It can be seen that we are close to 100\% uniform over all level sets for the interpolation experiment. 

% \begin{figure}[t]
%     \begin{center}
%         \includegraphics[width=0.8\columnwidth]{Figures/quantitative_analysis_NN_unsupervised_interpolation.png}
%     \end{center}
%     \caption{Interpolation Uniformity Analysis: The Figure analyzes the uniformity achieved by \newourmethod{} on intermediate level sets which consists of 4 second trajectory with 0.2 time discretization when the training consists of 0.4 discretozation. It can be observed that \newourmethod{} is uniform on all level sets during interpolating on intermediate level sets}
%     \label{fig:dubins_interpolation}
% \end{figure}

 

% \begin{figure}[!h]
%     \begin{center}
%         \includegraphics[width=0.8\columnwidth]{Figures/quantitative_analysis_NN_unsupervised_extrapolation.png}
%     \end{center}
%     \caption{Extrapolation Uniformity Analysis:  The Figure analyzes the uniformity achieved by \newourmethod{} on level sets  of 6 second trajectory with 0.2 discretization when trained with 4 second trajectory with 0.4 discretization. It can be observed that \newourmethod{} is uniform on all level sets including extrapolation to later level sets}
%     \label{fig:dubins_uniformity_extrapolation}
% \end{figure}

% \subsection{Coverage Analysis}  \label{sec: coverage_exp}

% In this experiment, we divide the configuration space into grid cells and calculate the number of grid cells covered by the sampled trajectories from the presented method and the baseline methods using the algorithm \ref{algo:coverage_metric}. Due to the near-exponential increase in the number of representative grid cells per level set as the number of trajectory samples grows, the coverage of later level sets appears comparatively low. To address this, we first report the coverage as a percentage of the total reachable space. Table \ref{tab:comparison_coverage} summarizes the comparison results and demonstrates that Neural C-Uniform outperforms the baseline methods, while following a similar trend to \prevapproach{}.


% \begin{algorithm}[h]
% \caption{Coverage Metric Calculation} \label{algo:coverage_metric}
% \KwIn{
%     \( \boldsymbol{\delta} \): The uniformity resolution of a grid cell;
    
%     \( g(x, \boldsymbol{\delta}) \): Function mapping a state $x$ to its grid cell in the configuration space, based on resolution $\boldsymbol{\delta}$;
     
%     \( \{R_t \mid t = 0, 1, 2, \dots, T\} \): Reachable cells for each level set \( t \);
 
%     \( X = \bigcup_{i=1}^N \{x_0^i, x_1^i, \dots, x_T^i\} \): Set of \( N \) trajectories;
% }
% \KwOut{
%     \( Cover_t \): Level set coverage percentage for each \( t \);
    
%     \( Cover \): Total coverage percentage across all level sets;
% }
% Initialize \( Unique_t = \emptyset \) for all \( t \).

% \For{each time step \( t = 0, 1, \dots, T \)}{
%     \For{each trajectory \( i = 1, 2, \dots, N \)}{
%        \For{each state \( x_t^i \) in trajectory \( i \) at time \( t \)}{
%             \( Unique_t \leftarrow Unique_t \cup \{g(x_t^i)\} \).
%         }
%     }
%     $Cover_t = \frac{|Unique_t|}{|R_t|} \times 100$
% }
% $Cover = \frac{\sum_{t=0}^T |Unique_t|}{\sum_{t=0}^T |R_t|} \times 100$

% \Return $Cover_t, Cover$
% \end{algorithm}
% Secondly, we compare the per-level-set coverage of methods under a fixed set of 10,000 trajectories while maintaining the same horizon and time discretization settings. This comparison also demonstrates similar trends, with Neural C-Uniform showcasing better performance than the baselines and aligning closely with \prevapproach{}. Figure \ref{fig:1d_uniformity} shows the comparisons, and it can be observed that \newourmethod{} outperforms all the approaches by 5\% on all level sets.






\subsection{Simulation Experiments} \label{sec: simulation}


In this experiment, we showcase the performance of our approach in various environmental settings. We compare our method's performance against the mentioned baselines, MPPI, and log-MPPI, on BARN dataset~\cite{barn}. Variance values both MPPI variants are $\Sigma = 0.3$, and their temperature value is fixed to $\lambda = 0.5$. This dataset focuses on the performance evaluation of cluttered environment navigations. The environments in the dataset are specifically designed to introduce challenging navigation scenarios, including local traps such as narrow passages and dead-end pockets. We use $Success\ Rate (SR)$ as the performance metric to evaluate the methods' performances. In Table~\ref{tab:combined_analysis}, we report the performance of the baselines and \newourmethod{} in 2 different time horizon settings. First, all methods are set to generate $2s$ long trajectories with the $0.2s$  time discretization. Finally, we showcase the exploration analysis under the $0.2s$  time discretization with an extended $3s$ time horizon.

% \subsubsection{Cost Function} The cost function $J$ is designed to guide motion planning by two objectives: the state obstacle cost $\mathcal{C}_{\text{obs}}(x_t)$, which penalizes states based on the local costmap values to avoid obstacles and the distance-to-goal cost $\mathcal{C}_{\text{goal}}(x_t, x_{\text{goal}})$, which encourages the trajectory to minimize the distance to the goal $x_{\text{goal}}$. The total cost $J$ is computed over a time horizon $T$, and the relative importance of obstacle avoidance and goal-reaching is controlled by a weighting factor $\lambda$. 

% The equation of the cost function $J$ for each trajectory is shown as follows:
% \begin{equation}
%     J^{\tau} = \sum_{t=0}^{T-1} \left( \lambda_{\text{obs}}\mathcal{C}_{\text{obs}}(x_t^{\tau}) + \lambda_{\text{goal}} \mathcal{C}_{\text{goal}}(x_t^{\tau}, x_{\text{goal}}) \right)    
% \end{equation}
% where a trajectory $\tau = F(x_{\text{curr}},U) =\{x_t^{\tau}\}_{t=0}^{T-1}$ and the initial state is equals to the current state $x_0^{T} = x_{\text{curr}}$.

% To compute $\mathcal{C}_{\text{obs}}(x_t^{\tau})$, we define it based on the collision conditions:

% \begin{equation}
%     \mathcal{C}_{\text{obs}}(x_t^{\tau}) =
%     \begin{cases}
%         \mathcal{C}_{\text{collision}}, & \text{if } \exists x_i^{\tau} \in \{x_i^{\tau}\}_{i=0}^{t-1} \text{ s.t. } x_i \text{ is in collision} \\
%         \mathcal{C}_{\text{local}}(x_t^{\tau}), & \text{otherwise}
%     \end{cases}
% \end{equation}
% where $\mathcal{C}_{\text{collision}}$ is the max collision cost, and         $\mathcal{C}_{\text{local}}(x_t^{\tau})$ calculates the cost of robot footprint of the state based on the local costmap.

% We define the goal cost function $\mathcal{C}_{\text{goal}}(x_t^{\tau}, x_{\text{goal}})$ as follows:

% \begin{equation}
% \begin{split}
% &\mathcal{C}_{\text{goal}}(x_t^{\tau}, x_{\text{goal}}) = \\
% &\begin{cases}
%     \mathcal{C}_{\text{distance}}, & \text{if } \exists x_i^{\tau} \in \{x_i^{\tau}\}_{i=0}^{t-1} \text{ s.t. } x_i \text{ is in collision} \\
%     ||x_t^{\tau} - x_{\text{goal}}||, & \text{otherwise}
% \end{cases}
% \end{split}
% \end{equation}
% where $\mathcal{C}_{\text{distance}}$ is the goal cost of the state where the collision happened along a trajectory $\tau$.



% $(\boldsymbol{\uparrow})$} 



% \subsubsection{BARN Dataset Result} We evaluate the performance of our method across all environments in the BARN dataset. Table~\ref{tab:combined_analysis} reports the success rates of each method for arbitrarily selected initial and goal positions with $10000$ sampled trajectories. Since the simulation operates in a noise-free setting, system propagations are deterministic.

% \renewcommand{\arraystretch}{1.5}
% \begin{table}[htbp]
% \centering
% \caption{Performance Analysis with Varying Time Horizons}
% % \caption{Performance Metrics, Interpolation, and Extrapolation Analysis}
% \begin{tabular}{l|c|c}
% % \toprule
% \hline
% \multicolumn{3}{c}{\textbf{Success Rate (\textbf{$\uparrow$})}} \\
% % \midrule
% \hline
% \textbf{Method} & \textbf{$T = 2s$} & \textbf{$T=3s$} \\
% % \midrule
% \hline
% \newourmethod  & 0.88 & \textbf{0.94} \\
% MPPI  & 0.77 & 0.81 \\
% log-MPPI & \textbf{0.90} & 0.93 \\
% % iCEM              & X & X \\
% \bottomrule
% \end{tabular}
% \label{tab:combined_analysis}
% \end{table}

% For $2s$ long trajectories, our approach and log-MPPI achieve comparable results, both outperforming standard MPPI. As the time horizon increases, the performance of all methods improves. However, with an extended time horizon, our method surpasses the baseline approaches. We now showcase some specific qualitative results for the simulations to present the scenario's where exploration \newourmethod{} is ne 

% \begin{figure*}[!h]
%     \begin{center}
%         \includegraphics[width=1.0\textwidth]{Figures/coverage_nn_c_uniform.png}
%     \end{center}
%     \caption{\textbf{Coverage:} The illustrated environment settings emphasize the importance of high coverage in trajectory sampling. A diverse set of trajectories allows Neural C-Uniform to effectively identify feasible navigation areas and improves its ability to avoid obstacles and reach the goal. In contrast, since neither MPPI variant could demonstrate good exploration of the configuration space in these environments, their solutions led to dead ends.}
%     \label{}
% \end{figure*}

% \begin{figure*}[!h]
%     \begin{center}
%         \includegraphics[width=1.0\textwidth]{Figures/long_horizon_nn_c_uniform.png}
%     \end{center}
%     \caption{\textbf{Long Horizon Sampling:}}
%     \label{}
% \end{figure*}

% \begin{figure*}[!h]
%     \begin{center}
%         \includegraphics[width=1.0\textwidth]{Figures/failure_nn_cuiniform.png}
%     \end{center}
%     \caption{\textbf{Failure Scenarios:} These results highlight the limitations of the proposed trajectory selection process. While the method effectively identifies lower-cost regions, the assumption that the minimum-cost trajectory at the current time $t$ leads to the goal can be misleading. In some cases, as shown with these two environment settings, the selected action may steer the system into a local trap and prevent successful navigation.}
%     \label{}
% \end{figure*}

\gtxt{FIG} provides qualitative insights into why MPPI variants yield different solutions compared to our method, while \gtxt{FIG} illustrates how extrapolating the time horizon influences the generated trajectories.



% One limitation of the previous method is its reliance on hyperparameters for optimization, which can make it computationally infeasible after some iterations. Specifically, it often leads to one of two scenarios:
% \begin{itemize}
%     \item Short horizons with small time steps, offering frequent updates but limited foresight.
%     \item Long horizons with large time steps, sacrificing resolution for extended predictions.
% \end{itemize}

% To address this, we introduce interpolation to increase the time-frequency while maintaining long horizons and extrapolation to extend the prediction horizon with minimal impact on time step size. This experiment quantifies the performance loss associated with interpolated and extrapolated models, highlighting the trade-offs and their practical significance.

% \subsection{Trajectory Smoothness}
% \begin{itemize}
%     \item Why is the smoothness important? 
%     \item How does it affect navigation in a complex environment?
%     \item How do we measure the smoothness of Trajectories? 
% \end{itemize}

\subsection{Real-World Experiments} \label{sec: real_world_exp}

We designed two different real-world environments to evaluate the capabilities of our algorithm.

\subsubsection{Cluttered Environment}

In this experiment, we compared our method against the baselines, MPPI and log-MPPI, using an F1Tenth vehicle in a cluttered environment. For mapping and localization, we utilized the SLAM Toolbox~\cite{Macenski2021} and Navigation2 (Nav2)~\cite{macenski2023survey} ROS2 packages. The SLAM Toolbox was used for map generation, while Nav2 handled localization and costmap generation based on LiDAR scan readings.

The experiment was conducted with three initial regions and a fixed goal region. For each initial position, we performed five trials for each method. Figure \ref{fig:real_trajectory_comparison} illustrates the experiment's environments and the generated trajectories. Additionally, we report each method's success rates and travel distances across different initial conditions.

% As a result, Neural C-Uniform achieved a higher success rate than the two baseline methods. It also produced shorter average trajectory lengths. Meanwhile, log-MPPI outperformed MPPI, demonstrating that diverse trajectory sampling helps identify feasible navigation regions more effectively.

 % - \yukangtxt{Placeholder text and figures here, yukang will add explanation for trajectory statistics and experiments setup}
 
I need to write a figure caption that explains the following: A Circular Motion: The 





==> sections/limitations.tex <==
\section{Limitations}

\begin{itemize}
    \item 
\end{itemize}

==> sections/old_texts.tex <==
\begin{figure}[!h]
    \begin{center}
        \includegraphics[width=1.0\columnwidth]{Figures/Runtime_vs_Planning.png}
    \end{center}
    \caption{Computational Cost Analysis: We analyze the time taken to determine probability by Maxflow \ourmethod{} where x-axis represents the planning horizon and y-axix represents the time taken for state-action probability computation. It can be seen that as the planning horizon increases the computational complexity keeps on increasing exponentially}
    \label{fig:dubins_comp}
\end{figure}

% Coverage Table

\begin{table*}[tbp]
    \centering
    \caption{\small Coverage Performance Comparison of MPPI, log-MPPI, Uniform Action Sampling, and \ourmethod~at Varying Sample Sizes. Each setting consists of 4-second trajectories with a time step of $0.2s$. Using Dubin's car dynamic with constant velocity $1 m/s$. The uniformity resolution for $x, y, \psi$ axes is set to $0.05m, 0.05m, 4.5^\circ$ respectively. Three covariance values are selected for different levels of exploration, where low, medium, and high variance corresponds to $0.03, 0.1, 0.3$ respectively.\vtxt{let's make this figure 1}}
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{c|ccc|ccc|c|c|c}
    \toprule
    % \textbf{\begin{tabular}[c]{@{}c@{}}Number of\\ Sampled Trajectories\end{tabular}} & \multicolumn{7}{c}{\textbf{Coverage Performance     $\boldsymbol{\uparrow}$}} \\
    \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Number of\\ Sampled \\ Trajectories\end{tabular}}} & \multicolumn{7}{c}{\textbf{Coverage Performance $ (\%) \boldsymbol{\uparrow}$}} \\

    \cmidrule(lr){2-9} 
    & \multicolumn{3}{c|}{\textbf{MPPI}} & \multicolumn{3}{c|}{\textbf{log-MPPI}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Uniform \\ Action\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Neural \\ C-Uniform \end{tabular}}} & \multirow{2}{*}{\textbf{\ourmethod }} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7}  
     & \textbf{Low} & \textbf{Medium} & \textbf{High} & \textbf{Low} & \textbf{Medium} & \textbf{High} \\
    \midrule
    500  &  0.11   &  0.42    &  1.96    &  0.34    &  2.03     &  3.79   & 3.16   & 4.13    & \textbf{5.01}  \\
    1000 &  0.12   &  0.50    &  2.72    &  0.38    &  2.69     &  6.02   & 4.80   & 7.00    & \textbf{9.08}  \\
    2500 &  0.12   &  0.59    &  3.67    &  0.44    &  3.79     &  10.4   & 7.35   & 13.09   & \textbf{18.95} \\
    5000 &  0.13   &  0.66    &  4.58    &  0.50    &  4.75     &  14.37  & 9.75   & 19.48   & \textbf{31.74} \\
    10000 & 0.14   &  0.74    &  5.47    &  0.55    &  5.81     &  19.36  & 12.58  & 27.11   & \textbf{49.79} \\
    25000 & 0.14   &  0.82    &  6.85    &  0.64    &  7.46     &  26.51  & 16.66  & 37.34   & \textbf{76.69} \\
    50000 & 0.14   &  0.92    &  7.97    &  0.71    &  8.81     &  32.02  & 20.01  & 44.53   & \textbf{91.50} \\

    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:comparison_coverage}
\end{table*}

% OLD HISTOGRAM UNIFORMITY ANALYSIS
\begin{figure*}[!h]
    \begin{center}
        \includegraphics[width=\textwidth]{Figures/uniformity_plots.png}
    \end{center}
    \caption{Uniformity Analysis:  \newourmethod{} learns to sample uniformly on all level sets. The X-axis represents the level sets for a 6-second time horizon with 0.2-second discretization. We test the uniformity performance of \newourmethod{} for both interpolation and extrapolation. The interpolation (blue) experiment focuses on training with a 4-second time horizon with 0.4-second discretization and testing with 0.2-second discretization which showcases the capability of \newourmethod{} to act as a high frequency controller. The extrapolation (orange) experiment focuses on training with a 4-second time horizon with 0.2-second discretization and testing on a 6-second horizon which shows the capability of \newourmethod{} to plan for longer horizons. It can be observed that \newourmethod{} is uniform on all level sets.}
    \label{fig:dubins_uniformity_analysis}
\end{figure*}

% COVERAGE METRIC ANALYSIS

\begin{figure}[!th]
    \begin{center}
        \includegraphics[width=1.0\columnwidth]{Figures/coverage_metric.png}
    \end{center}
    \caption{Coverage Metric Analysis: The Figure analyzes the coverage performance per level set of \newourmethod{} compared to baselines using 10000 trajectories. It can be seen that \newourmethod{} outperforms other approaches in terms of coverage metric by 5\% on every level set. \vtxt{this is obviously false! }}
    \label{fig:1d_uniformity}
\end{figure}


% OLD INTRO TEXTS
For example, in dynamically changing environments, an optimal trajectory may require a rare sequence of inputs, such as an evasive maneuver in response to sudden obstacle appearances.

--

% Fig.~\ref{fig:dubins_comp} demonstrates the exponential increase behavior and is a clear indication of the limitation in the scalability of the approach. 

% Besides the scalability issue, having grid-based representation also leads to some information loss about the finer details about the relation of configuration space and control inputs probabilities. 

% \begin{itemize}
%     \item State neural networks can learn an underlying continuous representation of the configuration space.
%     \item   Extending this work by training a neural network model under the supervision of representative grids and their corresponding action probabilities is not entirely straightforward. The network-flow-based optimization approach presented in that work focuses on determining action probabilities without enforcing smoothness over the C-space. As a result, adjacent cells may exhibit significantly different distributions due to the under-constrained nature of the problem.  
% \end{itemize}

--

Recent works in the domains like Robot Follow-Ahead~\cite{jiang2024mapawarehumanposeprediction} and pursuit- evasion~\cite{gonultas2024learningplaypursuitevasiondynamic} have showcased that neural networks have the ability to generate effective controls to perform the task such as human-trajectory generation and catching a evader. In our work, we look at the problem of can neural-network learn to generate the trajectories that uniformly covers the configuration space over time. In this way, a trained network can generate trajectories for longer time horizons and also function as a high-frequency controller. A straightforward method to train such a neural network model is to use the action probabilities of \ourmethod{} as supervision. However, this presents a challenge: the network-flow-based optimization approach presented in \ourmethod{} method focuses on determining action probabilities without enforcing smoothness over the C-space, which results in adjacent cells exhibiting significantly different distributions due to the under-constrained nature of the problem. 


% --- CEM METHODS FOR SBMPC related work 
Another important line of research in SBMPC explores the role of entropy in optimizing the sampling distributions to improve performance. The Cross-Entropy Method (CEM)~\cite{rubinstein1999cross} is a well-known method in SBMPC. Recent work also demonstrates its effectiveness for both improving the performance of other sampling-based motion planners~\cite{kobilarov2012cross}, and optimizing the policies~\cite{pourchot2018cem}. Recent advancements aim to adapt CEM for real-time decision-making. The DCEM~\cite{amos2020differentiable} method introduces differentiable versions of CEM, enabling gradient-based updates to improve its efficiency. More recently, the iCEM~\cite{pinneri2021sample} incorporates temporally correlated actions and memory mechanisms to achieve faster and more efficient planning.

% --- MPPI formulation with KL divergence
\begin{equation}\label{argmin_kl}
    \begin{split}
        \mathbf{U}_t^* & = \arg\min_{\mathbf{U}_t \in \mathcal{U}} \mathbb{E}_{\mathbf{V}_i \sim \mathbb{Q}} \left[ \mathbf{J}(\mathbf{X}, \mathbf{U}) \right] \\ 
                    & \approx \arg\min_{\mathbf{U}_t \in \mathcal{U}} \{ D_{\text{KL}}(\mathbb{Q}^* \parallel \mathbb{Q}) \}
    \end{split}
\end{equation}

% ----


\subsection{Sampling Based Model Predictive Control}
\label{sec:sbmpc_pre}
We provide related concepts and formulation of sampling-based model predictive control by reviewing the Information-Theoretic MPPI algorithm~\cite{williams2018information}. 

MPPI problem formulation also considers a generic robotic system similar to the one defined in Eq.~\ref{eq;kinematic_bicycle_model}. MPPI optimizes the action sequence $\mathbf{U} =(\mathbf{u}_t, \mathbf{u}_{t+1}, \dots, \mathbf{u}_{t+T})$ at a discrete time step $t$ with $T$ time horizon. The optimization problem is given as follows:

\begin{equation}\label{eq:opt_control}
    \begin{split}
        & \mathbf{U}_t^* = \arg\min_{\mathbf{U}_t \in \mathcal{U}} \mathbb{E}_{\mathbf{V} \sim q(V|U,\Sigma)} \left[ J(\statevec_0, \mathbf{V}) \right] \\
        & s.t.\quad J(\statevec_0, \mathbf{V}) = \phi(\statevec_{T})  + \sum_{t=0}^{T-1} \mathcal{L}(\statevec_t, \mathbf{v}_t)
    \end{split}
\end{equation}
where, $\mathbf{v}_t = \mathbf{u}_t + \epsilon$, and $\epsilon \sim \mathcal{N}(0,\Sigma)$. $q(V|U.\Sigma)$ is the probability density function of the probability distribution $\mathbb{Q}$ for noise-added control input sequence $\mathbf{V}$. The cost function $J$ is calculated by the terminal cost $\phi(\statevec_T)$ and the running stage cost $\mathcal{L}(\statevec_t, \mathbf{v}_t)$. The running cost is separated into two parts: the state cost $S$, and the input cost $\mathcal{A}$. Following this separation, \textit{Free Energy} of the system is defined as:
\vspace{-4pt}
\begin{equation}
\mathcal{F}(S,p, \statevec_0, \lambda) =  \text{log}\left( \mathbb{E}_{\mathbb{P}}\left[\text{exp}\left( -\frac{1}{\lambda} S(\mathbf{V})\right) \right] \right) 
\end{equation}
where $S(\mathbf{V})$ is the trajectory cost, $\lambda$ is a temperature parameter, and $\mathbb{P}$ is a base probability distribution. A key property of the free energy is that it provides a lower bound on the optimal cost. It can be shown as: 


\begin{equation}\label{eq:lower_bound_free}
    -\mathcal{F}(S,p, \statevec_0, \lambda) \leq \mathbb{E}_{\mathbb{Q}}[\frac{1}\lambda{}S(\mathbf{V})] + D_{KL}(\mathbb{Q}||\mathbb{P})
\end{equation}
where $\mathbb{Q}$ is a controlled distribution and its probability density is $q(\mathbf{V|\mathbf{U}, \Sigma})$. After assigning base distribution and defining the optimal distribution as: 
\begin{align}\label{eq:base_prob_opti}
    p(\mathbf{V}) & = q(\mathbf{V|\tilde{\mathbf{U}}, \Sigma}) \\
    q^*(\mathbf{V}) & \propto \text{exp}\left(-\frac{1}{\lambda}S(\mathbf{V})\right)p(\mathbf{V})
\end{align}
where the control input sequence $\tilde{\mathbf{U}}$ is used as a nominal input sequence for the probability density function $q$. Additionally, the optimal control input $q^*$ is defined as proportional to the $p$. After these definitions, the inequality in Eq.~\ref{eq:lower_bound_free} can be seen as optimizing the expected cost is equivalent to minimizing the KL divergence between the optimal trajectory distribution $\mathbb{Q}^*$ and a control policy $\mathbb{Q}$.
\begin{equation}\label{eq:argmin_kl}
    \mathbf{U}^* = \arg\min_{\mathbf{U \in \mathcal{U}}} D_{KL}(\mathbb{Q^*}||\mathbb{Q})
\end{equation}

After some algebraic transformations and using the importance sampling technique, the Eq.~\ref{eq:argmin_kl} can be derived as:
\begin{equation}\label{eq:opt_u_calc}
    \begin{split}
        & \mathbf{U}^* = \mathbb{E}_{\mathbb{Q}}\left[w(\mathbf{V})\mathbf{V}) \right] \\
        & w(\mathbf{V}) = \left(\frac{q^*(\mathbf{V})}{q(\mathbf{V}|\mathbf{U},\Sigma)} \right) = \left(\frac{q^*(\mathbf{V})}{p(\mathbf{V})} \right) \left(\frac{p(\mathbf{V})}{q(\mathbf{V}|\mathbf{U},\Sigma)} \right)
    \end{split}
\end{equation}
where $\mathbb{Q}$ is the controlled action probability distribution, and $\mathbf{U}^*$ represent the optimal action sequence for a given base distribution $\mathbb{P}$. For brevity, we direct readers to the cited paper~\cite{williams2018information} for the detailed derivation of the optimal control action sequence. In practice, Monte-Carlo approximation methods are used to estimate the control action sequence.

However, the assumption that both $p(\mathbf{V})$ and $q^*(\mathbf{V})$ are Gaussian introduces fundamental limitations in scenarios where the cost landscapes are highly nonconvex or multimodal. A single Gaussian distribution may fail to capture alternative low-cost trajectories if the cost function has multiple modes, potentially leading to suboptimal solutions as illustrated in Fig.~\ref{fig:drawback_illustration}. Additionally, in dynamically changing environments, the initial control mean may be far from the optimal mode. Gaussian perturbations might struggle to explore the correct region, causing MPPI to get stuck in local minima. These limitations highlight the need for enhanced exploration or methods to shift MPPI trajectories toward low-cost areas, ensuring that the search is conducted in the correct space. By introducing \newourmethod{} trajectory sampling, we aim to increase exploration and demonstrate how these trajectories can be incorporated into MPPI variants to enhance their performance.


% ----- 

\multirow{4}{*}{C-Uniform~\cite{poyrazoglu2024cuniformtrajectorysamplingfast}}  & \multirow{2}{*}{2500} & 0.05 & 1 & -  & 1 & -  & 1 & - & 1 & -  & 1 & - \\
    % \cmidrule(lr){3-13}
    & & 0.1 & 1 & -  & 1 & - & 1 & - & 1 & -  & 1 & - \\
    \cmidrule(lr){2-13}
    & \multirow{2}{*}{5000} & 0.05 & 1 & -  & 1 & -  & 1 &-  & 1 & - & 1 & - \\
    % \cmidrule{3-13}
    & & 0.1 & 1 & - & 1 & -  & 1 & -  & 1 & -  & 1 & - \\
    \midrule

    % ---

    % \begin{table}[htbp]
% \centering
% \caption{Performance Analysis of ...}
%  \begin{tabular}{l|c|c|c|c}
% % \toprule
% \hline
% \multicolumn{5}{c}{\textbf{Trajectories Statistics}} \\
% % \midrule
% \hline
% \textbf{Method} & \textbf{Success Rate\textbf{$\uparrow$}} & \textbf{Mean\textbf{$\downarrow$}} & \textbf{Median\textbf{$\downarrow$}} & \textbf{Range}\\ 
% % \midrule
% \hline
% \newourmethod   & \textbf{93\%} & \textbf{12.67} & \textbf{12.59} & 12.20-13.88\\
% MPPI            & 13\%          & 13.29          & 13.29          & 13.09-13.49\\
% log-MPPI        & 53\%          & 13.51          & 13.43          & 12.76-14.56\\
% % iCEM              & X & X \\
% \bottomrule
% \end{tabular}
% \label{tab:real_world_analysis}
% \end{table}
 
%  \begin{figure*}[h]
%     \centering
%     \subfloat[MPPI]{\includegraphics[width=0.32\textwidth]
%     {Figures/vanilla_mppi_cropped.pdf}}
%     \hfill
%     \subfloat[Log-MPPI]{\includegraphics[width=0.32\textwidth]{Figures/log_mppi_cropped.pdf}}
%     \hfill
%     \subfloat[\newourmethod{}]{\includegraphics[width=0.32\textwidth]{Figures/neural_cuniform_cropped.pdf}}
%     % \hfill
%     % \subfloat[\ourmethod]{\includegraphics[width=0.45\textwidth]{Figures/neural_cuniform_pdfcrop.pdf}}
%     \caption{Real-world trajectory visualization comparison in a cluttered corridor environment using F1Tenth. Our method \newourmethod{} shows the highest success rate 93\% compared to other MPPI variants. TODO: also add details experiments setup(dt, planning horizon, velocity, dynamic model}
%     \label{fig:real_trajectory_comparison}
% \end{figure*}

% \begin{figure}[!th]
%     \begin{center}
%         \includegraphics[width=0.5\columnwidth]{Figures/experiments_setup.jpg}
%     \end{center}
%     \caption{Real-world cluttered experiments environment setup, a narrow corridor with added obstacles.}
%     \label{fig:cluttered_experiment}
% \end{figure}
% To showcase the practical utility of our method, we designed an experimental environment in which a robot navigates toward arbitrarily selected target points while avoiding both static and dynamic obstacles.


% ---  MAYBE USED IN CONCLUSION
As mentioned earlier, other methods have similar mode-seeking behavior, such as optimizing reverse KL divergence to find one of the modes of cost distribution, as in~\cite{honda2024steinvariationalguidedmodel},~\cite{kobayashi2022real}. They rely on gradient calculation, which can introduce challenges, particularly in highly nonlinear cost landscapes where gradients may vanish or lead to convergence to suboptimal local modes. On the other hand, our \newourmethod{} trajectories cover the entire trajectory space uniformly. This increases the likelihood of generating trajectories near the global mode so that the MPPI trajectory sampling can be done around the lowest-cost region.



\textbf{System Specs:} All simulation experiments are conducted on a Ubuntu 24.04 platform. The computer is equipped with 24 cores Intel i9-13900HX, Nvidia GeForce RTX 4090 (16 GB memory), and 32 GB DDR5 RAM. Real-world experiments were conducted on the F1Tenth racer platform~\cite{o2020f1tenth}, which runs ROS2 \cite{doi:10.1126/scirobotics.abm6074} Foxy on Ubuntu 20.04 and is equipped with an Nvidia Jetson Xavier as the computing platform and a 2D LiDAR sensor (UST 10LX HOKUYO).
